PAC Reinforcement Learning with Rich Observations

We propose and study a new model for reinforcement learning with rich observations, generalizing contextual bandits to sequential decision making. These models require an agent to take actions based on observations (features) with the goal of achieving long-term performance competitive with a large set of policies. To avoid barriers to sample-efficient learning associated with large observation spaces and general POMDPs, we focus on problems that can be summarized by a small number of hidden states and have long-term rewards that are predictable by a reactive function class. In this setting, we design and analyze a new reinforcement learning algorithm, Least Squares Value Elimination by Exploration. We prove that the algorithm learns near optimal behavior after a number of episodes that is polynomial in all relevant parameters, logarithmic in the number of policies, and independent of the size of the observation space. Our result provides theoretical justification for reinforcement learning with function approximation.

==> proofs.tex <==
\section{Proof Sketch}
\label{sec:analysis}

For the proof sketch, we ignore logarithmic dependence on
$M,K,H,\epsilon$ and all dependence on $\delta$.  This considerably
simplifies the presentation without compromising the core ideas.  All
proof details are deferred to Appendix~\ref{app:full_proof}. For the
sketch, we recall our earlier notation $V^f(p,
\pi_f)$ in Equation~\ref{eqn:vfdef}.

%% One of the main components of the algorithm performs depth first search with a learning step and an exploration technique that prevents examining the exponentially large search tree. 
%% At a high level the algorithm aims to maintain only the regressors that approximate the $Q^\star$ function well, and it makes progress by discarding regressors that have a poor fit.
%% This elimination step is performed at each path $p$ visited by the depth first search, first by collecting samples from each of the direct descendants $p\circ a$ and forming Monte-Carlo estimates of the value function,
%% \begin{align*}
%% V^f(p \circ a, \pi_f) = \EE_{x \sim \dst{p\circ a}} f(x,\pi_f(x))
%% \end{align*}
%% for each $f$. We call these estimates $\hat{V}^f(p\circ a, \pi_f)$. 

%% With these estimates, we again use samples $(x,a,r)$ collected from $p$ with actions taken uniformly at random to estimate a notion of square loss,
%% \begin{align*}
%% R_p(f) = \EE_{(x,r) \sim \dst{p}, a \sim \textrm{Unif}(\Acal)} (f(x,a) - r(a) - \hat{V}^f(p\circ a - \pi_f))^2.
%% \end{align*}
%% Denote the empirical version of this risk with $\hat{R}_p(f)$.
%% The learning step is to eliminate regression functions that have large excess empirical risk. 
%% More precisely, we set,
%% \begin{align*}
%% \Fcal \gets \left\{f \in \Fcal : \hat{R}_p(f) \le \min_{f' \in \Fcal} \hat{R}_p(f') + \Delta\right\},
%% \end{align*}
%% for a tolerance parameter $\Delta$.

%% As we are navigating the search space, we use the set of surviving regressors to guide exploration using what we call a \emph{consensus test}. 
%% At a path $p$, this test is performed by forming monte-carlo estimates for,
%% \begin{align*}
%% \EE_{x\sim \dst{p}} f(x,\pi_f(x)) - g(x,\pi_g(x))
%% \end{align*}
%% for all pairs of surviving functions $f,g \in \Fcal$. 
%% We report that consensus is reached if all of the estimates are at most some tolerance $\epstest$, which depends on the level $h$.
%% %% collecting $n$ observations $\{x_i\}_{i=1}^n$ from $p$ (over the course of $n$ trajectories) and verifying that,
%% %% \begin{align*}
%% %% \left|\frac{1}{n}\sum_{i=1}^nf(x_i,\pi_f(x_i)) - g(x_i,\pi_g(x_i))\right| \le \epstest \forall \textrm{ surviving } f,g,
%% %% \end{align*}
%% %% for a carefully chosen threshold $\epstest$ that depends on the level $h$. 
%% The insight here is that $V^\star(p) = \EE_{x \sim p}f^\star(x,\pi_{f^\star}(x))$ so that if $f^\star \in\Fcal$, this test ensures that all remaining regressors accurately predict the value of the state reached after rolling in according to $p$. 

%% The depth first search uses consensus tests to avoid exploring the entire search tree. 
%% When the search arrives at a path $p$, we only recursively explore the descendants $p\circ a$ if consensus has \emph{not} been reached at those states. 
%% As we saw above, this condition is sufficient for successfully running the regression step at $p$.
%% Moreover, the second guarantee from the elimination step shows that, if we have already trained on the (observation, reward) distribution induced by the path $p\circ a$, then this test returns \texttt{true} with high probability, thus implicitly performing a state equality test at a level needed by the class $\Fspace$.
%% The first property ensures that we invoke the training mechanism properly, while the second property implies that we avoid exploring the entire search tree.

%% The first phase of the algorithm is one execution of this depth first search started from the root of the search tree.
%% This suffices to estimate the optimal value $V^\star$.

\textbf{Analysis of DFS:}
%% Let $\phi = \frac{\epsilon}{320H^2\sqrt{K}}$ and set $\tau_h = 20h\sqrt{K}\phi$ for each $h$. 
Consider running the elimination step (step~\ref{algline:elim} in
Algorithm~\ref{alg:dfs_learn} at some path $p$ with $h$ actions to go
and set $\tau_h = 20h\sqrt{K}\phi$.  Our analysis shows that after
this step, all surviving regressors agree on the value of this state
and take near-optimal actions at this state.  We also ensure that
$f^\star$ is never eliminated.  The guarantee requires two
preconditions involving the surviving functions to hold at the
descendant states.  The \emph{estimation precondition} is that for all
$f\in \Fcal, a \in \Acal$, we have $|\hat{V}^f(p\circ a,\pi_f) -
V^f(p\circ a, \pi_f)| \le \phi$.  The \emph{bias precondition} is that
for all pairs $f,g\in\Fcal$ and all $a \in \Acal$ we have
$|V^f(,p\circ a, \pi_f) - V^g(p\circ a, \pi_g)| \le \tau_{h-1}$.  If
both preconditions are met, we prove that after collecting
$\log(\Fsize)/\phi^2$ samples and performing the elimination step at
$p$,
\begin{enumerate}
\item $f^\star$ is retained by the algorithm.
\item $|V^f(p,\pi_f) - V^g(p,\pi_g)| \le 10\phi\sqrt{K} + \tau_{h-1} = 20(h-1/2)\sqrt{K}\phi$ for all surviving $f,g$.
\item $\EE_{x\sim p}f^\star(x,\pi_{f^\star}(x)) - f^\star(x,\pi_f(x)) \le 10\phi\sqrt{K} + 2\tau_{h-1}$ for all surviving $f$.
\end{enumerate}
The proof here is driven by the fact that $f^\star$ is realizable for its regression target in the square loss problem in Eq.~\ref{eq:td_sq_loss}.
This follows from the definition of $\qs$, which implies that for any state $s$ generating observation $x$,
\begin{align}
f^\star(x,a) &= \EE_{r \sim \dst{s|x}}r(a) + V(\Trans(s,a),\pi_{f^\star})  = \EE_{r \sim \dst{s|x}} r(a) + \EE_{x'\sim \dst{\Trans(s,a)}} f^\star(x',\pi_{f^\star}(x')). \label{eq:f_consistency}
\end{align}
Thus $f^\star$ is consistent between its estimate at the current state $s$ and the future state $s' = \Trans(s,a)$.
Our regression problem is a finite sample version of this identity. 
Moreover, the bias and estimation preconditions ensure that all the targets used for each regressor are very close, which enables us to guarantee that all regressors make similar predictions.

Before discussing how these claims are used, we first verify the preconditions.
First, we are guaranteed that the estimation precondition is always satisfied, because we collect $\ntest=\order(\log(\Fsize)/\phi^2)$ samples at each descendant during execution of \statelearned.
Secondly, an inductive argument using the definition of $\tau_h$ and the second claim here ensures that the bias precondition is always met. 

We use the second claim to control the sample complexity while we use the third claim to prove the PAC guarantee.
To build intuition for the PAC-guarantee, suppose that the elimination step has been executed at all states.
Then inductively for any surviving $f$, we have,
\begin{align*}
V^\star - V(\pi_f) &= \EE_{x\sim \dst{\treeroot}} f^\star(x,\pi_{f^\star}(x)) - f^\star(x,\pi_f(x)) + f^\star(x,\pi_f(x)) - r(\pi_f(x)) - V(\pi_f(x), \pi_f)\\
& \le O(2\tau_H) + \EE_{x\sim \dst{\treeroot}} \EE_{x' \sim \dst{\pi_f(x)}} f^\star(x',\pi_{f^\star}(x')) - f^\star(x',\pi_f(x')) \le O(2\sum_{h=1}^H\tau_h)
\end{align*}
This is the overall suboptimality bound and plugging in our definition of $\tau_h$ we see that it is $O(H^2\sqrt{K}\phi)$. 
With our setting of $\phi$, this bound is at most $\epsilon$. 

To bound the sample complexity, we argue that the elimination step is executed on each state at most once. 
If we have executed the elimination step on a state distribution, then the second claim above, the choice of $\epstest$, and a elementary deviation bound, guarantee that the consensus test returns true every time we visit this state. 
%% This also guarantees that the bias precondition is met every time we run the elimination step.
This requires collecting $O(\frac{\log(\Fsize)}{K\phi^2})$ for each consensus test.

While the consensus test only requires $O(\frac{\log(\Fsize)}{K\phi^2})$ samples, the estimation precondition requires that we collect $O(\frac{\log(\Fsize)}{\phi^2})$ samples at each of the descendant states.
This means that each time we execute the elimination step, we collect $O(\frac{K\log(\Fsize)}{\phi^2})$ samples in total, also accounting for the consensus tests at the direct descendants. 
Since we run the elimination step at most $MH$ times, this gives an overall sample complexity of $O(\frac{K^2MH^5\log(\Fsize)}{\epsilon^2})$. 

\textbf{On-Demand Exploration:}
The only missing piece of the above argument is that in proving the PAC-guarantee, we assumed that the elimination step was executed at \emph{all} states. 
Given that we use consensus tests to truncate the DFS we may not visit all states, so this assumption may not hold.
However, we use a more refined version of the inequality used to prove the PAC bound. 
If $L$ is the set of states on which we have executed the elimination step, we show that for any surviving $f$,
\begin{align}
V^\star - V(\pi_f) \le O(\sum_{h=1}^H\tau_h) + \PP[\pi_f \textrm{ exits } L] \label{eqn:on_demand_regret}
\end{align}

The PAC guarantee follows trivially here, since the procedure only terminates when it finds a near-optimal policy.
Moreover, Eq.~\eqref{eqn:on_demand_regret} confirms that this procedure makes rapid progress because a policy can only be highly suboptimal if it exits $L$ with substantial probability. 
Specifically every time the algorithm finds a policy $\pi_f$ that is more than $\epsilon$ suboptimal, we have $\PP[\pi_f \textrm{ exits} L] \ge \Omega(\epsilon)$ and a Chernoff bound shows that with $O(1/\epsilon)$ paths we must find a new, unlearned state with high probability. 
By calling the elimination step on these $O(1/\epsilon)$ paths, we ensure that the set $L$ grows by at least one on every iteration. 
Since $|L| \le MH$, this bounds the total number of iterations of the on-demand exploration component. 

With an amortized counting argument, we show that On-Demand exploration introduces a multiplicative factor of $H/\epsilon$ into the sample complexity bound.
This happens because we may perform up to $MH$ iterations of On-Demand exploration, and each one involves executing the elimination component on all $H$ prefixes of $O(1/\epsilon)$ paths.
Inside the DFS routine, elimination is never called on the same state twice, so the total number of elimination calls is $O\left(\frac{MH^2}{\epsilon} + MH\right)$.
Combining with the sample complexity for each elimination step proves the theorem. 

